Edge-preserving Near-light Photometric Stereo with Neural Surfaces

This paper presents a near-light photometric stereo method that faithfully preserves sharp depth edges in the 3D reconstruction. Unlike previous methods that rely on finite differentiation for approximating depth partial derivatives and surface normals, we introduce an analytically differentiable neural surface in near-light photometric stereo for avoiding differentiation errors at sharp depth edges, where the depth is represented as a neural function of the image coordinates. By further formulating the Lambertian albedo as a dependent variable resulting from the surface normal and depth, our method is insusceptible to inaccurate depth initialization. Experiments on both synthetic and real-world scenes demonstrate the effectiveness of our method for detailed shape recovery with edge preservation.

==> figures/exp/initial_shape_eval_two_column.tex <==
\makebox[0.16\textwidth]{\footnotesize Ours} 
\makebox[0.4\textwidth]{\footnotesize LB20~\cite{logothetis2020cnn}}
\makebox[0.4\textwidth]{\footnotesize \quad QD18~\cite{queau2018led}}
\\
\makebox[1\textwidth]{\includegraphics[ width=1\textwidth]{images/depth_init/depth_init.pdf}}
\\
%\makebox[0.5\textwidth]{\includegraphics[ width=0.5\textwidth]{images/depth_init/ours_N_err_table.pdf}}
%\\
%\makebox[0.5\textwidth]{\includegraphics[ width=0.5\textwidth]{images/depth_init/ours_Z_err_table.pdf}}
%\\
%{\includegraphics[ width=0.232\textwidth]{images/depth_init/ours_N_err_table_m.pdf}}
%{\includegraphics[ width=0.232\textwidth]{images/depth_init/ours_Z_err_table_m.pdf}}

\begin{tabular}{@{}cc@{}}
	{\includegraphics[ width=0.5\textwidth]{images/depth_init/ours_N_err_table_m.pdf}}
	&{\includegraphics[ width=0.5\textwidth]{images/depth_init/ours_Z_err_table_m.pdf}}
\end{tabular}




==> figures/exp/non_lambert_eval.tex <==
	\resizebox{1\textwidth}{!}{\begin{tabular}{@{}c@{}@{}c@{}|@{}c@{}@{}c@{}|@{}c@{}@{}c@{}}
			\hline
			\multicolumn{2}{c|}{(A) Lambertian Diffuse} & \multicolumn{2}{c}{(B) Oren-Nayar Diffuse} & \multicolumn{2}{|c}{(C) Specular Reflectance} \\
			\multicolumn{2}{c|}{$\sigma_d = 0$, $\sigma_s = 0$} & \multicolumn{2}{c|}{$\sigma_d = 1.0$ , $\sigma_s = 0$} & \multicolumn{2}{c}{$\sigma_d = 0$ , $\sigma_s = 0.3$} \\
			\hline
			{\includegraphics[ width=\imgsize\textwidth]{images/non_lambert/lambert.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/non_lambert/analytical_N_mae_err_0.33.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/non_lambert/diffuse.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/non_lambert/ours_N_mae_err_2.44.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/non_lambert/spec.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/non_lambert/ours_N_mae_err_2.39.png}}
			\begin{minipage}{0.013\textwidth} \centering
				\vspace{-5.2em} \makebox[0.6\textwidth]{ $\; 5^{\circ}$}\\ \vspace{-0em}
				\makebox[0.5\textwidth]{}\includegraphics[width=0.7\linewidth]{images/color_bar} \\ \vspace{-0.4em}
				\makebox[0.5\textwidth]{ $\; 0^{\circ}$}\\
			\end{minipage}
		\\ \hline
		\end{tabular}}
	\resizebox{1\textwidth}{!}{
	\begin{tabular}{@{}c@{}c@{}}
		{\includegraphics[ width=0.24\textwidth]{images/non_lambert/ours_diffuse.pdf}}
		&{\includegraphics[ width=0.24\textwidth]{images/non_lambert/ours_spec.pdf}}
	\end{tabular}
	}



%
%
%%
%\begin{tabular}{c@{}@{}c}
%	\resizebox{0.7\textwidth}{!}{
%		\LARGE
%		\begin{tabular}{c|c|c}
%			\hline
%			(A) Lambertian Diffuse & (B) Oren-Nayar Diffuse & (C) Specular Reflectance \\
%			$\sigma_d = 0$, $\sigma_s = 0$ & $\sigma_d = 1.0$ , $\sigma_s = 0$ & $\sigma_d = 0$ , $\sigma_s = 0.3$ \\
%			\hline
%			{\includegraphics[ width=\imgsize\textwidth]{images/non_lambert/lambert.png}}
%			&{\includegraphics[ width=\imgsize\textwidth]{images/non_lambert/diffuse.png}}
%			&{\includegraphics[ width=\imgsize\textwidth]{images/non_lambert/spec.png}}
%			\\
%			{\includegraphics[ width=\imgsize\textwidth]{images/non_lambert/analytical_N_mae_err_0.33.png}}
%			&{\includegraphics[ width=\imgsize\textwidth]{images/non_lambert/ours_N_mae_err_2.44.png}}
%			&{\includegraphics[ width=\imgsize\textwidth]{images/non_lambert/ours_N_mae_err_2.39.png}}
%			\begin{minipage}{0.013\textwidth} \centering
%				\vspace{-5.2em} \makebox[0.6\textwidth]{ $ 5$}\\ \vspace{-0em}
%				\makebox[0.5\textwidth]{}\includegraphics[width=0.8\linewidth]{images/color_bar} \\ \vspace{-0.4em}
%				\makebox[0.5\textwidth]{ $ 0$}\\
%			\end{minipage}
%			\\ \hline
%		\end{tabular}
%	}
%	&
%	\resizebox{0.3\textwidth}{!}{
%	\begin{tabular}{c}
%	\resizebox{0.3\textwidth}{!}{\includegraphics[ width=0.32\textwidth]{images/non_lambert/ours_diffuse.pdf}}
%	\\
%	\resizebox{0.3\textwidth}{!}{\includegraphics[ width=0.32\textwidth]{images/non_lambert/ours_spec.pdf}}
%	\end{tabular}
%	}
%
%\end{tabular}

==> figures/exp/non_lambert_eval_half.tex <==
	\resizebox{1\textwidth}{!}{
		\LARGE
		\begin{tabular}{ccc}
			\hline
			{(A) Lambertian Diffuse} & {(B) Oren-Nayar Diffuse} & {(C) Specular Reflectance} \\
			{$\sigma_d = 0$, $\sigma_s = 0$} & {$\sigma_d = 1.0$ , $\sigma_s = 0$} & {$\sigma_d = 0$ , $\sigma_s = 0.3$} \\
			\hline
			{\includegraphics[ width=0.4\textwidth]{images/non_lambert/lambert.png}}
			&{\includegraphics[ width=0.4\textwidth]{images/non_lambert/diffuse.png}}
			&{\includegraphics[ width=0.4\textwidth]{images/non_lambert/spec.png}}\\
			&{\includegraphics[ width=0.4\textwidth]{images/non_lambert/analytical_N_mae_err_0.33.png}}
			&{\includegraphics[ width=0.4\textwidth]{images/non_lambert/ours_N_mae_err_2.44.png}}
			&{\includegraphics[ width=0.4\textwidth]{images/non_lambert/ours_N_mae_err_2.39.png}}
			\begin{minipage}{0.013\textwidth} \centering
				\vspace{-5.2em} \makebox[0.6\textwidth]{ $ 5$}\\ \vspace{-0em}
				\makebox[0.5\textwidth]{}\includegraphics[width=0.8\linewidth]{images/color_bar} \\ \vspace{-0.4em}
				\makebox[0.5\textwidth]{ $ 0$}\\
			\end{minipage}
		\\ \hline
		\end{tabular}
	}
	\resizebox{1\textwidth}{!}{
	\begin{tabular}{@{}c@{}c@{}}
		{\includegraphics[ width=0.24\textwidth]{images/non_lambert/ours_diffuse.pdf}}
		&{\includegraphics[ width=0.24\textwidth]{images/non_lambert/ours_spec.pdf}}
	\end{tabular}
	}

==> figures/exp/real_quantative_eval.tex <==
	\resizebox{\textwidth}{!}{
	\begin{threeparttable}
		\begin{tabular}[t]{cccccc!{\vrule width 0.8pt}cccccc}
			\noalign{\hrule height 1.2pt}
			& \multicolumn{5}{c!{\vrule width 0.8pt}}{Normal estimation error~(MAngE)}  &  \multicolumn{6}{c}{Depth estimation error~(MAbsE)}  \\ 
       		Method & LB17~\cite{logothetis2017semi} & QD18~\cite{queau2018led} & SM20~\cite{santo2020deep} & LB20~\cite{logothetis2020cnn} & Ours & LB17~\cite{logothetis2017semi} & QD18~\cite{queau2018led} & SM20~\cite{santo2020deep} & LB20~\cite{logothetis2020cnn} & Ours & Ours~(S)\tnote{1} 
       		\\
       		\noalign{\hrule height 1.2pt}
			{\sc Ball} & \underline{9.77} & 12.12 & 25.42 & 12.43 & \textbf{9.02 }& \underline{0.81 }& 2.5 & 5.5 & \textbf{0.67} & 20.92 & 1.18  \\ 
			{\sc Buddha} & \underline{11.5}  & 14.07 & 19.17 & \textbf{10.73} & 11.95 & 4.67 & 9.28 & 5.53 & \textbf{3.27} & 45.29 & \underline{4.40}  \\ 
			{\sc Bunny} & 20.15 & 13.73 & 12.5 & \underline{8.15} & \textbf{8.13 }& 7.51 & 7.06 & 6.02 & \underline{2.49} & 27.58 & \textbf{1.49}  \\ 
			{\sc Die} & 11.95 & 13.77 & \textbf{5.23 }& 6.55 & \underline{6.32} & 4.58 & 5.91 & \underline{2.76} & 4.44 & 25.41 & \textbf{2.37} \\ 
			{\sc Hippo} & 15.42 & 18.51 & 23.12 & \textbf{7.75} & \underline{9.75} & 3.19 & 6.8 & 7.04 & \textbf{1.82} & 24.91 &  \underline{1.97}  \\ 
			{\sc House} & 29.69 & 30.63 & \underline{28.02} & 30.03 & \textbf{27.54 }& 6.99 & 8.02 & \underline{6.15}& 9.14 & 28.47 & \textbf{5.61}  \\ 
			{\sc Owl} & 13.77 & 14.74 & 13.08 & \underline{12.39} & \textbf{8.38} & 3.64 & 5.83 & 3.75 & \underline{3.44} & 28.71 & \textbf{2.74}  \\ 
			{\sc Jar} & 10.56 & 15.66 & 9.27 & 8.6 & \textbf{4.25} & 6.56 & 16.87 & 6.09 & \textbf{3.86} & 34.61 & \underline{3.96}  \\ 
			{\sc Queen} & 13.05 & 13.16 & 16.62 & \underline{10.96} & \textbf{9.96} & \textbf{1.89} & 6.92 & 3.91 & \underline{1.94} & 33.69 & 2.20  \\ 
			{\sc Squirrel} & 15.93 & \underline{14.06} & 14.07 & 15.12 & \textbf{12.78} & 1.82 & 2.55 & 2.81 & \textbf{1.01}& 34.34 & \underline{1.55}  \\ 
			{\sc Bowl} & 12.5 & 11.19 & 12.44 & \textbf{8.78} & \underline{9.97} & 4.37 & 6.48 & 5.22 & \textbf{2.80} & 31.16 & \underline{3.45}  \\ 
			{\sc Tool} & \underline{15.1} & 16.12 & 17.42 & 17.05 & \textbf{14.56} & \textbf{3.25} & 6.69 & \underline{4.68} & 5.90 & 67.64 & 6.57  \\ 
			\noalign{\hrule height 1.2pt} 
%			\rowcolor{lightgray}
			Avg (partial)\tnote{2} & 14.95 & 15.65 & 16.36 & \underline{12.38} & \textbf{11.05} & 4.11 & 7.08 & 4.96 & \underline{3.40} & 33.56 & \textbf{3.12}  \\ 
			\noalign{\hrule height 1.2pt} 
			{\sc Bell} & 28.25 & 25.8 & \textbf{9.5 }& \underline{14.74} & 39.34 & 4.45 & 12.03 & \underline{1.9} & \textbf{1.53} & 55.76 & 39.02  \\ 
			{\sc Cup} & 30.76 & 37.63 & \textbf{14.22} & \underline{23.35} & 59.31 & 2.67 & 4.83 & \textbf{1.62} & \underline{2.04} & 466.38 & 112.69  \\ 
			Avg (all)\tnote{3}  & 17.03 & 17.94 & \underline{15.72} & \textbf{13.33} & 36.56 & \underline{4.02} & 7.27 & 4.5 & \textbf{3.17} & 185.23 & 51.61 \\ 
			\noalign{\hrule height 1.5pt}
		\end{tabular}
		\begin{tablenotes}[para]
			\item[1] Scaled depth estimates of our method\\
			\item[2] Average error of the first $12$ objects\\
			\item[3] Average error of all the $14$ objects
		\end{tablenotes}
	\end{threeparttable}
}


==> figures/exp/supp_synthetic_comp_normal.tex <==
	\resizebox{1\textwidth}{!}{
		\large
		\begin{tabular}{@{}c:c@{}@{}c@{}@{}c@{}@{}c@{}@{}c@{}}
			GT shape &QD18~\cite{queau2018led}   &LB20~\cite{logothetis2020cnn} & SM20~\cite{santo2020deep}   &MQ16~\cite{mecca2016single} & Ours  \\
			{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/normals.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/QD18_2974.1501808166504/N_est_QD18.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/LB20_2974.1501808166504/N_est_LB20.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/SM20_2974.1501808166504/N_est_SM20.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/MQ16_2974.1501808166504/N_est_MQ16.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/Ours/N_est_Ours.png}}
			\\
			{\sc Tent} & 5.41  & 2.29  & 9.99  & 10.99  & 1.72  
			\\
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/QD18_2974.1501808166504/QD18_N_mae_err_5.41.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/LB20_2974.1501808166504/LB20_N_mae_err_2.29.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/SM20_2974.1501808166504/SM20_N_mae_err_9.99.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/MQ16_2974.1501808166504/MQ16_N_mae_err_10.99.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/Ours/Ours_N_mae_err_1.72.png}}
			\begin{minipage}{0.02\textwidth} \centering
				\vspace{-5.5em} \makebox[0.5\textwidth]{ $\;\; 15^{\circ}$}\\ \vspace{-0em}
				\makebox[0.5\textwidth]{}\includegraphics[width=0.7\linewidth]{images/color_bar} \\ \vspace{-0.4em}
				\makebox[0.5\textwidth]{ $\;\; 0^{\circ}$}\\
			\end{minipage}\\
			{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/normals.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/QD18_2641.799211502075/N_est_QD18.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/LB20_2641.799211502075/N_est_LB20.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/SM20_2641.799211502075/N_est_SM20.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/MQ16_2641.799211502075/N_est_MQ16.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/Ours/N_est_Ours.png}}
			\\
			{\sc Bunny} & 1.66 & 3.94  & 7.43  & 8.54  & 0.33 
			\\
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/QD18_2641.799211502075/QD18_N_mae_err_1.66.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/LB20_2641.799211502075/LB20_N_mae_err_3.94.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/SM20_2641.799211502075/SM20_N_mae_err_7.43.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/MQ16_2641.799211502075/MQ16_N_mae_err_8.54.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/Ours/Ours_N_mae_err_0.33.png}}
			\begin{minipage}{0.02\textwidth} \centering
				\vspace{-5.5em} \makebox[0.5\textwidth]{ $\;\; 15^{\circ}$}\\ \vspace{-0em}
				\makebox[0.5\textwidth]{}\includegraphics[width=0.7\linewidth]{images/color_bar} \\ \vspace{-0.4em}
				\makebox[0.5\textwidth]{ $\;\; 0^{\circ}$}\\
			\end{minipage}\\
			{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/normals.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/QD18_2741.1582469940186/N_est_QD18.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/LB20_2741.1582469940186/N_est_LB20.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/SM20_2741.1582469940186/N_est_SM20.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/MQ16_2741.1582469940186/N_est_MQ16.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/Ours/N_est_Ours.png}}
			\\
			{\sc Buddha} & 7.84  & 4.44 & 12.19  & 10.44  & 2.11 
			\\
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/QD18_2741.1582469940186/QD18_N_mae_err_7.84.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/LB20_2741.1582469940186/LB20_N_mae_err_4.44.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/SM20_2741.1582469940186/SM20_N_mae_err_12.19.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/MQ16_2741.1582469940186/MQ16_N_mae_err_10.43}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/Ours/Ours_N_mae_err_2.11.png}}
			\begin{minipage}{0.02\textwidth} \centering
				\vspace{-7.5em} \makebox[0.5\textwidth]{ $\;\; 15^{\circ}$}\\ \vspace{-0em}
				\makebox[0.5\textwidth]{}\includegraphics[width=0.7\linewidth]{images/color_bar} \\ \vspace{-0.4em}
				\makebox[0.5\textwidth]{ $\;\; 0^{\circ}$}\\
			\end{minipage}\\
		\end{tabular}	
	}

==> figures/exp/supp_synthetic_comp_shape.tex <==
	\resizebox{1\textwidth}{!}{
		\large
		\begin{tabular}{@{}c:c@{}@{}c@{}@{}c@{}@{}c@{}@{}c@{}}
			GT shape &QD18~\cite{queau2018led}   &LB20~\cite{logothetis2020cnn} & SM20~\cite{santo2020deep}   &MQ16~\cite{mecca2016single} & Ours  \\
			{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/13_pyramid/shape_vis_supp/crop/shape_gt_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/13_pyramid/shape_vis_supp/crop/shape_QD18_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/13_pyramid/shape_vis_supp/crop/shape_LB20_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/13_pyramid/shape_vis_supp/crop/shape_SM20_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/13_pyramid/shape_vis_supp/crop/shape_MQ16_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/13_pyramid/shape_vis_supp/crop/shape_ours_crop.png}}
			\\
			{\sc Tent} & 0.055  & 0.093   & 0.371 & 0.111  & \textbf{0.003}
			\\
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/QD18_2974.1501808166504/QD18_Z_mabs_err_5.52e-02.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/LB20_2974.1501808166504/LB20_Z_mabs_err_9.35e-02.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/SM20_2974.1501808166504/SM20_Z_mabs_err_3.71e-01.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/MQ16_2974.1501808166504/MQ16_Z_mabs_err_1.11e-01.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/Ours/Ours_Z_mabs_err_2.68e-03.png}}
			\begin{minipage}{0.02\textwidth} \centering
				\vspace{-5.5em} \makebox[0.5\textwidth]{ $\;\; 0.3\,$m}\\ \vspace{-0em}
				\makebox[0.5\textwidth]{}\includegraphics[width=0.7\linewidth]{images/color_bar} \\ \vspace{-0.4em}
				\makebox[0.5\textwidth]{ $\; 0\;$m}\\
			\end{minipage}\\
			{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/04_bunny/shape_vis_supp/crop/shape_gt_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/04_bunny/shape_vis_supp/crop/shape_QD18_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/04_bunny/shape_vis_supp/crop/shape_LB20_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/04_bunny/shape_vis_supp/crop/shape_SM20_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/04_bunny/shape_vis_supp/crop/shape_MQ16_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/04_bunny/shape_vis_supp/crop/shape_ours_crop.png}}
			\\
			{\sc Bunny} &  0.024 &  0.031   & 0.058 & 0.060  & \textbf{0.003}
			\\
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/QD18_2641.799211502075/QD18_Z_mabs_err_2.41e-02.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/LB20_2641.799211502075/LB20_Z_mabs_err_3.08e-02.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/SM20_2641.799211502075/SM20_Z_mabs_err_5.79e-02.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/MQ16_2641.799211502075/MQ16_Z_mabs_err_6.00e-02.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/Ours/Ours_Z_mabs_err_2.73e-03.png}} 
			\begin{minipage}{0.02\textwidth} \centering
				\vspace{-5.5em} \makebox[0.5\textwidth]{ $\;\; 0.3\,$m}\\ \vspace{-0em}
				\makebox[0.5\textwidth]{}\includegraphics[width=0.7\linewidth]{images/color_bar} \\ \vspace{-0.4em}
				\makebox[0.5\textwidth]{ $\; 0\;$m}\\
			\end{minipage}\\
			{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/17_buddha/shape_vis_supp/crop/shape_gt_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/17_buddha/shape_vis_supp/crop/shape_QD18_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/17_buddha/shape_vis_supp/crop/shape_LB20_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/17_buddha/shape_vis_supp/crop/shape_SM20_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/17_buddha/shape_vis_supp/crop/shape_MQ16_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/17_buddha/shape_vis_supp/crop/shape_ours_crop.png}}
			\\
			{\sc Buddha} & 0.071 & 0.129  & 0.149  & 0.097  & \textbf{0.009}
			\\
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/QD18_2741.1582469940186/QD18_Z_mabs_err_7.09e-02.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/LB20_2741.1582469940186/LB20_Z_mabs_err_1.29e-01.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/SM20_2741.1582469940186/SM20_Z_mabs_err_1.49e-01.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/MQ16_2741.1582469940186/MQ16_Z_mabs_err_9.72e-02.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/Ours/Ours_Z_mabs_err_9.00e-03.png}} 
			\begin{minipage}{0.02\textwidth} \centering
				\vspace{-7.5em} \makebox[0.5\textwidth]{ $\;\; 0.3\,$m}\\ \vspace{-0em}
				\makebox[0.5\textwidth]{}\includegraphics[width=0.7\linewidth]{images/color_bar} \\ \vspace{-0.4em}
				\makebox[0.5\textwidth]{ $\; 0\;$m}\\
			\end{minipage}\\
		\end{tabular}	
	}

==> figures/exp/synthetic_comp_one_column.tex <==
	\resizebox{0.5\textwidth}{!}{
		\LARGE
		\begin{tabular}{@{}c:c@{}@{}c@{}@{}c:c@{}@{}c@{}@{}c@{}}
			GT shape
			&\multicolumn{3}{c}{3D shape estimation}   &\multicolumn{3}{:c}{Depth absolute error} \\
			{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/13_pyramid/shape_vis_new3/crop/shape_gt_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/13_pyramid/shape_vis_new3/crop/shape_QD18_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/13_pyramid/shape_vis_new3/crop/shape_LB20_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/13_pyramid/shape_vis_new3/crop/shape_ours_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/QD18_2974.1501808166504/QD18_Z_mabs_err_5.52e-02.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/LB20_2974.1501808166504/LB20_Z_mabs_err_9.35e-02.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/Ours/Ours_Z_mabs_err_2.68e-03.png}}\\
			{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/04_bunny/shape_vis_new3/crop/shape_gt_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/04_bunny/shape_vis_new3/crop/shape_QD18_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/04_bunny/shape_vis_new3/crop/shape_LB20_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/04_bunny/shape_vis_new3/crop/shape_ours_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/QD18_2641.799211502075/QD18_Z_mabs_err_2.41e-02.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/LB20_2641.799211502075/LB20_Z_mabs_err_3.08e-02.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/Ours/Ours_Z_mabs_err_2.73e-03.png}} 
			\begin{minipage}{0.013\textwidth} \centering
				\vspace{-5.5em} \makebox[0.5\textwidth]{ $\; 0.1$}\\ \vspace{-0em}
				\makebox[0.5\textwidth]{}\includegraphics[width=0.9\linewidth]{images/color_bar} \\ \vspace{-0.4em}
				\makebox[0.5\textwidth]{ $\; 0$}\\
			\end{minipage}\\
			{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/17_buddha/shape_vis_new3/crop/shape_gt_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/17_buddha/shape_vis_new3/crop/shape_QD18_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/17_buddha/shape_vis_new3/crop/shape_LB20_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth]{images/data_compare_syn/17_buddha/shape_vis_new3/crop/shape_ours_crop.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/QD18_2741.1582469940186/QD18_Z_mabs_err_7.09e-02}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/LB20_2741.1582469940186/LB20_Z_mabs_err_1.29e-01.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/Ours/Ours_Z_mabs_err_9.00e-03.png}}
			\\
			&QD18~\cite{queau2018led}   &LB20~\cite{logothetis2020cnn} & Ours 			&QD18~\cite{queau2018led}   &LB20~\cite{logothetis2020cnn} & Ours\\
		\end{tabular}	
	}
	\resizebox{0.5\textwidth}{!}{
		\LARGE
		\begin{tabular}{@{}c:c@{}@{}c@{}@{}c:c@{}@{}c@{}@{}c@{}}
			GT Normal
			&\multicolumn{3}{c}{Surface normal estimation}   &\multicolumn{3}{:c}{Surface normal angular error} 
			\\
			{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/normals.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/LB20_2974.1501808166504/N_est_LB20.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/QD18_2974.1501808166504/N_est_QD18.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/Ours/N_est_Ours.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/QD18_2974.1501808166504/QD18_N_mae_err_5.41.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/LB20_2974.1501808166504/LB20_N_mae_err_2.29.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/Ours/Ours_N_mae_err_1.72.png}}
			\\
			{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/normals.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/QD18_2641.799211502075/N_est_QD18.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/LB20_2641.799211502075/N_est_LB20.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/QD18_2641.799211502075/QD18_N_mae_err_1.66.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/Ours/N_est_Ours.png}}			
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/LB20_2641.799211502075/LB20_N_mae_err_3.94.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/Ours/Ours_N_mae_err_0.33.png}}
			\begin{minipage}{0.013\textwidth} \centering
				\vspace{-5.5em} \makebox[0.5\textwidth]{ $\; 10$}\\ \vspace{-0em}
				\makebox[0.5\textwidth]{}\includegraphics[width=0.9\linewidth]{images/color_bar} \\ \vspace{-0.4em}
				\makebox[0.5\textwidth]{ $\; 0$}\\
			\end{minipage}\\
			{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/normals.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/QD18_2741.1582469940186/N_est_QD18.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/LB20_2741.1582469940186/N_est_LB20.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/Ours/N_est_Ours.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/QD18_2741.1582469940186/QD18_N_mae_err_7.84.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/LB20_2741.1582469940186/LB20_N_mae_err_4.44.png}}
			&{\includegraphics[ width=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/Ours/Ours_N_mae_err_2.11.png}}
			\\
			&QD18~\cite{queau2018led}   &LB20~\cite{logothetis2020cnn} & Ours 			&QD18~\cite{queau2018led}   &LB20~\cite{logothetis2020cnn} & Ours\\
		\end{tabular}	
	}

==> figures/exp/synthetic_data_large.tex <==
	\resizebox{1.0\textwidth}{!}{
		\LARGE
		\begin{tabular}{@{}c@{}@{}c@{}@{}c@{}@{}c@{}@{}c@{}@{}c@{}@{}c:c@{}@{}c@{}@{}c@{}@{}c@{}@{}c@{}@{}c@{}}
			\raisebox{2.8em}{\rotatebox{90}{GT}}
			& {\includegraphics[ height=\imgsize\textwidth]{images/data_compare_syn/13_pyramid/shape_vis_new3/crop/shape_gt_crop.pdf}}
			& {\includegraphics[ height=\imgsize\textwidth]{images/data_compare_syn/04_bunny/shape_vis_new3/crop/shape_gt_crop.pdf}}
			& {\includegraphics[ height=\imgsize\textwidth]{images/data_compare_syn/17_buddha/shape_vis_new3/crop/shape_gt_crop.pdf}}
			& \multicolumn{3}{c}{\makebox[0.1\textwidth]{}\hspace{-3em}\makebox[0.02\textwidth]{$0\,{\rm mm} \qquad$}\includegraphics[width=0.25\linewidth]{images/color_bar_h} \makebox[0.02\textwidth]{$ \qquad 100\,{\rm mm}$}}
			& {\includegraphics[ height=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/normals.png}}
			& {\includegraphics[ height=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/normals.png}}
			& {\includegraphics[ height=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/normals.png}}
			& \multicolumn{3}{c}{\makebox[0.1\textwidth]{}\hspace{-3em}\makebox[0.02\textwidth]{$0^{\circ} \quad$}\includegraphics[width=0.25\linewidth]{images/color_bar_h} \makebox[0.02\textwidth]{$ \quad 10^{\circ}$}}
			\\
			\raisebox{1.2em}{\rotatebox{90}{QD18~\cite{queau2018led}}}
			& 			{\includegraphics[ height=\imgsize\textwidth]{images/data_compare_syn/13_pyramid/shape_vis_new3/crop/shape_QD18_crop.pdf}}
			&			{\includegraphics[ height=\imgsize\textwidth]{images/data_compare_syn/04_bunny/shape_vis_new3/crop/shape_QD18_crop.pdf}}
			&			{\includegraphics[ height=\imgsize\textwidth]{images/data_compare_syn/17_buddha/shape_vis_new3/crop/shape_QD18_crop.pdf}}
			&			{\includegraphics[ height=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/QD18_2974.1501808166504/QD18_Z_mabs_err_5.52e-02.png}}
			&			{\includegraphics[ height=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/QD18_2641.799211502075/QD18_Z_mabs_err_2.41e-02.png}}
			&			{\includegraphics[ height=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/QD18_2741.1582469940186/QD18_Z_mabs_err_7.09e-02}}
			&			{\includegraphics[ height=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/QD18_2974.1501808166504/N_est_QD18.png}}
			&           {\includegraphics[ height=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/QD18_2641.799211502075/N_est_QD18.png}}
			&			{\includegraphics[ height=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/QD18_2741.1582469940186/N_est_QD18.png}}
			&			{\includegraphics[ height=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/QD18_2974.1501808166504/QD18_N_mae_err_5.41.png}}
			&			{\includegraphics[ height=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/QD18_2641.799211502075/QD18_N_mae_err_1.66.png}}
			&           {\includegraphics[ height=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/QD18_2741.1582469940186/QD18_N_mae_err_7.84.png}}
			\\
			\raisebox{1.2em}{\rotatebox{90}{LB20~\cite{logothetis2020cnn}}}
			&			{\includegraphics[ height=\imgsize\textwidth]{images/data_compare_syn/13_pyramid/shape_vis_new3/crop/shape_LB20_crop.pdf}}
			&			{\includegraphics[ height=\imgsize\textwidth]{images/data_compare_syn/04_bunny/shape_vis_new3/crop/shape_LB20_crop.pdf}}
			&			{\includegraphics[ height=\imgsize\textwidth]{images/data_compare_syn/17_buddha/shape_vis_new3/crop/shape_LB20_crop.pdf}}
			&			{\includegraphics[ height=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/LB20_2974.1501808166504/LB20_Z_mabs_err_9.35e-02.png}}
			&			{\includegraphics[ height=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/LB20_2641.799211502075/LB20_Z_mabs_err_3.08e-02.png}}
			&			{\includegraphics[ height=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/LB20_2741.1582469940186/LB20_Z_mabs_err_1.29e-01.png}}
			&			{\includegraphics[ height=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/LB20_2974.1501808166504/N_est_LB20.png}}
			&			{\includegraphics[ height=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/LB20_2641.799211502075/N_est_LB20.png}}
			&			{\includegraphics[ height=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/LB20_2741.1582469940186/N_est_LB20.png}}
			&			{\includegraphics[ height=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/LB20_2974.1501808166504/LB20_N_mae_err_2.29.png}}
			&			{\includegraphics[ height=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/LB20_2641.799211502075/LB20_N_mae_err_3.94.png}}
			&			{\includegraphics[ height=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/LB20_2741.1582469940186/LB20_N_mae_err_4.44.png}}
			\\			
			\raisebox{2.2em}{\rotatebox{90}{Ours}}		
			&{\includegraphics[ height=\imgsize\textwidth]{images/data_compare_syn/13_pyramid/shape_vis_new3/crop/shape_ours_crop.pdf}}
			&{\includegraphics[ height=\imgsize\textwidth]{images/data_compare_syn/04_bunny/shape_vis_new3/crop/shape_ours_crop.pdf}}
			&{\includegraphics[ height=\imgsize\textwidth]{images/data_compare_syn/17_buddha/shape_vis_new3/crop/shape_ours_crop.pdf}}
			&{\includegraphics[ height=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/Ours/Ours_Z_mabs_err_2.68e-03.png}}
			&{\includegraphics[ height=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/Ours/Ours_Z_mabs_err_2.73e-03.png}} 
			&{\includegraphics[ height=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/Ours/Ours_Z_mabs_err_9.00e-03.png}}
			&{\includegraphics[ height=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/Ours/N_est_Ours.png}}
			&{\includegraphics[ height=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/Ours/N_est_Ours.png}}
			&{\includegraphics[ height=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/Ours/N_est_Ours.png}}
			&{\includegraphics[ height=\imgsize\textwidth, trim={65px 65px 65px 65px},clip]{images/data_compare_syn/13_pyramid/Ours/Ours_N_mae_err_1.72.png}}
			&{\includegraphics[ height=\imgsize\textwidth, trim={10px 0px 40px 33px},clip]{images/data_compare_syn/04_bunny/Ours/Ours_N_mae_err_0.33.png}}
			&{\includegraphics[ height=\imgsize\textwidth, trim={112px 23px 112px 40px},clip]{images/data_compare_syn/17_buddha/Ours/Ours_N_mae_err_2.11.png}}
			\\
			& \multicolumn{3}{c}{GT / Est. shapes} & \multicolumn{3}{c}{Depth absolute error} & \multicolumn{3}{c}{GT / Est. surface normal} & \multicolumn{3}{c}{Surface normal angular error}
		\end{tabular}	
	}

==> figures/intro/diff_comp.tex <==
%\resizebox{0.5\textwidth}{!}{
%	\centering
%	\scriptsize
	\begin{threeparttable}
		\begin{tabular}{cc}
			\toprule
			Discrete surface model
			& Neural surface model
			\\
			\midrule
			\includegraphics[width=0.5\textwidth]{figures/intro/diff.pdf}
			& \includegraphics[width=0.5\textwidth]{figures/intro/analytical.pdf} 
			\\
				\vspace{-2em}
				\\
		\bottomrule
		\end{tabular}
	\end{threeparttable}	
%}

%
%	\centering
%\scriptsize
%\begin{threeparttable}
%	\begin{tabular}{c|c|c}
%		\Xhline{2\arrayrulewidth}
%		Discrete surface model
%		&
%		\includegraphics[width=0.2\textwidth]{figures/intro/finite2.pdf}
%		&
%		\makecell[l]{
%			\parbox[l]{0.2\textwidth}{\begin{equation*}
%					\mathcal{Z}(u) = \begin{cases}
%						1 & u \in  \{u_i, u_{i+1}\} \\
%						0 & u \in  \{u_{i-1}, u_{i-2}\}
%					\end{cases}
%					\label{eq:discrete_repre}
%					\end{equation*}}
%		\\
%		\parbox[l]{0.2\textwidth}{\begin{equation*}
%				\left.\frac{\partial \mathcal{Z}(u)}{\partial u}\right|_{u=u_i} \approx 
%				\frac{z_{i+1} - z_{i-1}}{2\Delta u} \hspace{1.5em}
%				\label{eq:finite_diff}
%		\end{equation*}}
%		}
%		\\
%		Neural surface model
%		&
%		\includegraphics[width=0.2\textwidth]{figures/intro/parametric2.pdf}
%		&
%		\makecell[l]{
%			\parbox[l]{0.2\textwidth}{\begin{equation*}
%				\mathcal{Z}(u) = \mathcal{Z}(u; \bm{\theta}) 
%				\label{eq:analytical_repre}
%		\end{equation*}}
%		\\
%		\parbox[l]{0.2\textwidth}{\begin{equation*}
%				\frac{\partial \mathcal{Z}(u)}{\partial u} = \frac{\partial \mathcal{Z}(u; \bm{\theta})}{\partial u}
%				\label{eq:analytical_diff}
%		\end{equation*}}
%		}
%	
%%		& Neural surface model
%%		\\
%%		\Xhline{\arrayrulewidth}
%%		\includegraphics[width=0.2\textwidth]{figures/intro/finite2.pdf}
%%		& \includegraphics[width=0.2\textwidth]{figures/intro/parametric2.pdf} \\
%%		Discrete image coordinate & Continuous image plane \\
%%		\Xhline{\arrayrulewidth}
%%		\hspace{-3.5em}
%%		\resizebox{.15\textwidth}{!}{
%%			\footnotesize
%%			\parbox[l]{0.2\textwidth}{\begin{eqnarray}
%%					\mathcal{Z}(u) = \begin{cases}
%%						1 & u \in  \{u_i, u_{i+1}\} \\
%%						0 & u \in  \{u_{i-1}, u_{i-2}\}
%%					\end{cases}
%%					\label{eq:discrete_repre}
%%		\end{eqnarray}}}
%%		&
%%		\hspace{-1em}
%%		\resizebox{.15\textwidth}{!}{
%%			\footnotesize
%%			\parbox[l]{0.2\textwidth}{\begin{equation*}
%%					\mathcal{Z}(u) = \mathcal{Z}(u; \bm{\theta}) 
%%					\label{eq:analytical_repre}
%%			\end{equation*}}
%%		} 
%%		\\
%%		\Xhline{\arrayrulewidth}
%%		\hspace{-5em}
%%		\quad
%%		\resizebox{.15\textwidth}{!}{
%%			\footnotesize
%%			\parbox[l]{0.2\textwidth}{\begin{eqnarray}
%%					\left.\frac{\partial \mathcal{Z}(u)}{\partial u}\right|_{u=u_i} \approx 
%%					\frac{z_{i+1} - z_{i-1}}{2\Delta u} \hspace{1.5em}
%%					\label{eq:finite_diff}
%%		\end{eqnarray}}}
%%		&
%%		\hspace{-1em}
%%		\resizebox{.15\textwidth}{!}{
%%			\footnotesize
%%			\parbox[l]{0.2\textwidth}{\begin{equation*}
%%					\frac{\partial \mathcal{Z}(u)}{\partial u} = \frac{\partial \mathcal{Z}(u; \bm{\theta})}{\partial u}
%%					\label{eq:analytical_diff}
%%		\end{equation*}}} \\
%%		\multicolumn{1}{c|}{Finite difference} & \multicolumn{1}{c}{Analytical derivative}\\
%%		\Xhline{2\arrayrulewidth}
%	\end{tabular}
%\end{threeparttable}

==> figures/intro/diff_comp2.tex <==
\resizebox{0.5\textwidth}{!}{
	\centering
	\large
	\begin{threeparttable}
		\begin{tabular}{l|l|c}
			\Xhline{2\arrayrulewidth}
			\multicolumn{1}{c|}{Surface with sharp edge}
			& \multicolumn{1}{c|}{Discrete surface model}
			& Neural surface model
			\\
			\Xhline{\arrayrulewidth}
			{\includegraphics[width=0.3\textwidth]{figures/intro/gt2.pdf}}
			& \includegraphics[width=0.3\textwidth]{figures/intro/finite2.pdf}
			& \includegraphics[width=0.3\textwidth]{figures/intro/parametric2.pdf} \\
			\Xhline{\arrayrulewidth}
					\qquad
			\resizebox{.15\textwidth}{!}{
			\parbox[l]{0.17\textwidth}{\begin{equation*}
				\mathcal{Z}(u) = \begin{cases}
						1 & u \geq 0 \\
						0 & u < 0
				\end{cases}
			\end{equation*}}}
			&
			\resizebox{.15\textwidth}{!}{
			\parbox[l]{0.17\textwidth}{\begin{eqnarray}
				\mathcal{Z}(u) = \begin{cases}
					1 & u \in  \{u_i, u_{i+1}\} \\
					0 & u \in  \{u_{i-1}, u_{i-2}\}
				\end{cases}
			\label{eq:discrete_repre}
			\end{eqnarray}}}
			&
			\hspace{-1em}
			\resizebox{.15\textwidth}{!}{
			\parbox[l]{0.17\textwidth}{\begin{equation*}
					\mathcal{Z}(u) = \mathcal{Z}(u; \bm{\theta}) 
			\label{eq:analytical_repre}
			\end{equation*}}
			} 
		\\
		\Xhline{\arrayrulewidth}
		\hspace{-1em}
			\qquad
		\resizebox{.15\textwidth}{!}{
			\parbox{0.17\textwidth}{\begin{equation*}
					\frac{\partial \mathcal{Z}(u)}{\partial u} = \begin{cases}
						0 & u \neq 0 \\
						{\rm N.A.} & u = 0
					\end{cases}
		\end{equation*}
	\vspace{-1.5em}}}
		&  
		\resizebox{.15\textwidth}{!}{
			\parbox[l]{0.17\textwidth}{\begin{eqnarray}
			\left.\frac{\partial \mathcal{Z}(u)}{\partial u}\right|_{u=u_i} \approx 
		 \frac{z_{i+1} - z_{i-1}}{2\Delta u} \hspace{1.5em}
		 \label{eq:finite_diff}
		\end{eqnarray}}}
		&
		\hspace{-1em}
		\resizebox{.15\textwidth}{!}{
			\parbox[l]{0.17\textwidth}{\begin{equation*}
					\frac{\partial \mathcal{Z}(u)}{\partial u} = \frac{\partial \mathcal{Z}(u; \bm{\theta})}{\partial u}
					\label{eq:analytical_diff}
		\end{equation*}}} \\
		 & \multicolumn{1}{c|}{Finite difference} & \multicolumn{1}{c}{Analytical derivative}\\
		\Xhline{2\arrayrulewidth}
		\end{tabular}
	\end{threeparttable}
	}

==> figures/intro/diff_comp3.tex <==
\resizebox{0.5\textwidth}{!}{
	\centering
	\begin{threeparttable}
		\begin{tabular}{l|c}
			\Xhline{2\arrayrulewidth}
			\multicolumn{1}{c|}{Discrete surface model}
			& Neural surface model
			\\
			\Xhline{\arrayrulewidth}
			\includegraphics[width=0.3\textwidth]{figures/intro/finite2.pdf}
			& 
			\resizebox{.15\textwidth}{!}{
				\parbox[l]{0.17\textwidth}{\begin{eqnarray}
						\mathcal{Z}(u) = \begin{cases}
							1 & u \in  \{u_i, u_{i+1}\} \\
							0 & u \in  \{u_{i-1}, u_{i-2}\}
						\end{cases}
						\label{eq:discrete_repre}
			\end{eqnarray}}}
		\end{tabular}
	\end{threeparttable}	}

==> figures/intro/diff_comp_stair_neural.tex <==
\resizebox{1\textwidth}{!}{
	\centering
	\begin{threeparttable}
		\begin{tabular}{ccc}
			\toprule
			\makecell[c]{\textbf{GT} \\ \textbf{surface}}
			\makecell[l]{
				\parbox[l]{0.3\textwidth}{\begin{equation*}
						\mathcal{Z}(u, v) = \begin{cases}
							1 & u>0, v>0, \\
							0 & {\rm Others}
						\end{cases}
			\end{equation*}}}
			& \makecell[c]{\textbf{Discrete surface} \\ \textbf{representation}}  
			\makecell[l]{
				\parbox[l]{0.3\textwidth}{\begin{equation*}
						z_\V{p} = \begin{cases}
							1 & \V{p} \in \Omega_1, \\
							0 & \V{p} \in \Omega_0 
						\end{cases}
			\end{equation*}}}
			& \makecell[c]{\textbf{Analytical surface} \\ \textbf{representation}} 
						\makecell[l]{
				\parbox[l]{0.3\textwidth}{\begin{equation*}
						z_\V{p} = \mathcal{Z}(u, v; \bm{\theta})
			\end{equation*}}}
			\\
			\midrule
			\includegraphics[width=0.5\textwidth]{figures/intro/gt_stair.pdf}
			& \includegraphics[width=0.5\textwidth]{figures/intro/finite_stair.pdf}
			& \includegraphics[width=0.5\textwidth]{figures/intro/sigmoid_stair.pdf} 
			\\
			GT derivative
			& 
			Finite difference approximation
			&
			Analytical derivative
			\\
			\makecell[l]{
						\parbox[l]{0.5\textwidth}{\begin{equation*}
					\nabla z_{\V{p}} =  \begin{bmatrix}
						\frac{\partial z_\V{p}}{ \partial u}, 
						\frac{\partial z_\V{p}}{ \partial v}
					\end{bmatrix}^\top
					=  \begin{bmatrix}
						0 \\
						0
					\end{bmatrix}
			\end{equation*}}}
			&
%			\makecell[c]{Finite \\ difference}
			\makecell[l]{
			\parbox[l]{0.5\textwidth}{\begin{equation*}
				 \nabla z_{\V{p}} \approx  \begin{bmatrix}
				 	 \frac{z_{\V{u}+} - z_{\V{u}-}}{ 2 \Delta u},
 				 	 \frac{z_{\V{v}+} - z_{\V{v}-}}{ 2 \Delta v}
				 \end{bmatrix}^\top
			 =  \begin{bmatrix}
			 	0 \\
			 	0.5
			 \end{bmatrix}
			\end{equation*}}}
			&
			\makecell[l]{
				\parbox[l]{0.5\textwidth}{\begin{equation*}
						\nabla z_{\V{p}} = 
						 \begin{bmatrix}
							\frac{\partial  \mathcal{Z}(u, v; \bm{\theta})}{\partial  u},
							\frac{\partial  \mathcal{Z}(u, v; \bm{\theta})}{\partial  v}
						\end{bmatrix}^\top 
						\approx
					 \begin{bmatrix}
							0 \\
							0
						\end{bmatrix}
			\end{equation*}}}
		\\
		\bottomrule
		\end{tabular}
	\end{threeparttable}	
}



==> figures/intro/motivation.tex <==
\resizebox{0.5\textwidth}{!}{
	\centering
	\large
	\begin{threeparttable}
		\begin{tabular}{c|c|c}
			\Xhline{2\arrayrulewidth}
			Surface with sharp edge
			& \makecell[c]{Discrete surface model \\ (Finite difference)}
			& \makecell[c]{Analytical surface model \\ (Analytical derivative)}\\
			\hline
			\includegraphics[width=0.3\textwidth]{figures/intro/gt2.pdf}
			& \includegraphics[width=0.3\textwidth]{figures/intro/finite2.pdf}
			& \includegraphics[width=0.3\textwidth]{figures/intro/parametric2.pdf} \\
			\Xhline{\arrayrulewidth}
		\end{tabular}
	\end{threeparttable}
	}

==> figures/intro/teaser2.tex <==
%\makebox[0.01\textwidth]{} 
\makebox[0.15\textwidth]{GT Surface} 
\makebox[0.15\textwidth]{QD18~\cite{queau2018led}} 
\makebox[0.15\textwidth]{Ours} 
\\ 
%\raisebox{3.4em}{\rotatebox[origin=t]{90}{\sc Sphere}}
%\includegraphics[width = 0.15\textwidth]{images/teaser/Sphere/crop/shape_crop.png}
%\includegraphics[width = 0.15\textwidth]{images/teaser/Sphere/crop/QD18_crop.png}
%\includegraphics[width = 0.15\textwidth]{images/teaser/Sphere/crop/Ours_crop.png}
%\\ 
%\raisebox{2.5em}{\rotatebox[origin=t]{90}{\sc Pyramid}}
\includegraphics[width = 0.15\textwidth]{images/teaser/pyramid/crop/crop_zoomin/shape_crop.png}
\includegraphics[width = 0.15\textwidth]{images/teaser/pyramid/crop/crop_zoomin/QD18_crop.png}
\includegraphics[width = 0.15\textwidth]{images/teaser/pyramid/crop/crop_zoomin/Ours_crop.png}
\\
\vspace{-1em}
